Resource Adequacy and Capacity Procurement: Metrics and Decision Support Analysis

Resource adequacy studies typically use standard metrics such as Loss of Load Expectation and Expected Energy Unserved to quantify the risk of supply shortfalls. This paper critiques present approaches to adequacy assessment and capacity procurement in terms of their relevance to decision maker interests, before demonstrating alternatives including risk-averse metrics and visualisations of wider risk profile. This is illustrated with results for a Great Britain example, in which the risk profile varies substantially with the installed capacity of wind generation. This paper goes beyond previous literature through its critical discussion of how current practices reflect decision maker interests; and how decision making can be improved using a broader range of outputs available from standard models.

==> junk.tex <==
%\subsubsection{Model of available conventional capacity}

%\cjd{Cut most of this}

%Available conventional generation at time $t$, $X_t$, is modelled as the sum of individual generating units' availabilities. In many studies including in GB, conventional generators are assumed to be either fully available or unavailable, and in almost all studies availabilities of different units are typically assumed to be independent of each other and of all other variables.

%For the non-sequential model, it is necessary only to specify an availability probability for each unit, and then the distribution of the aggregate can be constructed by convolution\footnote{The most efficient way to do this in principle is by Fast Fourier Transform. However, in practice this is usually not needed as a good code working in capacity-space will run fast enough -- it is helpful to round all capacities to the nearest MW, and then use integer arithmetic where relevant.}. 

%For the sequential model, a stochastic process must be specified -- the standard approach is to use a 2 state Markov birth-death process for each unit. This however is questionable, and in particular there is no  reason to think that the repair process should be Markovian -- Markov is more natural for the failure process, perhaps with a non-constant failure rate.

%\subsubsection{Data for conventional units}

%Even making the assumption of independence between units, data for estimating conventional plant properties can be problematic. In GB, National Grid ESO only have access to historic data on \emph{whether} plant was unavailable and not \emph{why}; this does not provide a good basis for estimating the probability that a unit is broken down, as the unavailable time might include times when a unit is simply switched off.

%In N American, there is central reporting of availability data to the Generation Availability Data System run by the N American Electricity Reliability Corporation, which publishes public summary statistics. There are still complications associated with using these data, for instance:
%\begin{itemize}
%    \item If a unit is switched off, there is no direct observation of its mechanical availability state.
%    \item When a unit returns to service after repair, one sees when it \emph{was} repaired, not when it \emph{could} have been repaired if particularly needed
%\end{itemize}

%There is also a possibility that failure rates of conventional generation are much elevated during periods of extreme temperature. Sinnott Murphy has done work on this using N American data -- however even then there are very limited data to explore the most extreme temperature, and trends as a function of temperature might not extrapolate if new failure modes are seen at the most extreme temperatures.

%\subsubsection{Possible decision analysis work within Turing 2.0 project and MUGM}

%\emph{This section is included here as it has in common with the rest of this section that it is written for people within these two projects. It would in other ways more logically sit as a conclusion.}

%The next section cites the standard `EEU times VOLL' monetisation of shortfall risk.

%with a given probability derived from historic data, and . Within the examples presented, risk indices that depend on the distribution of $Z_t$ may then be calculated by convolving the distributions of $X_t$ and $D'_t$. However, a time-sequential model would in general be needed to consider technologies such as storage that link time periods in the calculations, even when only expected value indices such as EEU and LOLE are evaluated.

\begin{figure}[h!]
    \centering
    \begin{subfigure}{.24\textwidth}
    \includegraphics[width=\textwidth]{optimal-lole-vs-alpha-0.0.pdf}
    \caption{Wind capacity: 0 GW}
    \label{fig:contours-0-wc}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
    \includegraphics[width=\textwidth]{optimal-lole-vs-alpha-24600.0.pdf}
    \caption{Wind capacity: 24 GW}
    \label{fig:contours-24-wc}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
    \includegraphics[width=\textwidth]{optimal-lole-vs-alpha-40700.0.pdf}
    \caption{Wind capacity: 41 GW}
    \label{fig:contours-40-wc}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
    \includegraphics[width=\textwidth]{optimal-lole-vs-alpha-71000.0.pdf}
    \caption{Wind capacity: 71 GW}
    \label{fig:contours-71-wc}
    \end{subfigure}
     \caption{Optimal procured capacity $x^*$ as a function of the risk aversion parameter $\alpha$ and CONE/VOLL.}
    \label{fig:ratio-vs-alpha}
\end{figure}

This figure does however illustrate how calculation results vary as a function of the risk aversion $\alpha$, the CONE/VOLL ratio, and the installed wind capacity. In particular, as capacity becomes cheaper relative to the monetisation of shortfalls the capacity procured increases; and as the wind capacity increases, the capacity procured increases, which will be explored later when the probability distribution of energy unserved is displayed. 
%-- this would also be an issue if one plots a Pareto frontier in $x$-CVaR space. It is notable however that the capacity-to-procure exhibits only very weak dependence on the installed wind capacity, which suggests that this CVaR-based analysis is not (at least for our GB example) incorporating any differences in risk profile at different wind penetrations. The next section will reveal why this is -- as the penetration of wind generation increases in our numerical experiment, the risk profile does indeed change, but not in a way that will be captured by CVaR.

%\emph{I am not sure whether here we have much to add in commentary, or whether it's simply a case of demonstrating that `numbers go in, numbers come out', and observing that the one does indeed see a difference in results at different risk aversions. It would be possible to consider alternative risk averse metrics, and to discuss in more detail how this can be used in decision analysis.}

%\cjd{Need to discuss further what example to use. We could provide the Pareto frontier for a range of $\alpha$, with the caveat that these are not directly comparable due to CVaRs at different $alpha$ not being directly comparable -- or it might be possible to use as the primary example here calculating EFC of the wind fleet for a version of the example comparable with the later visualisations.}
